When is more search useful? An Empirical Study of Search Utility in Quality-Aware Decoding for Machine Translation

Quality-Aware Decoding (QAD) improves machine translation through test-time scaling, generating multiple candidate translations and selecting the final output with a quality-aware decoder. Usually the same candidate budget N is spent on every source sentence, assuming that all inputs require the same amount of search. We show that this assumption does not hold and that the quality gain obtained from additional candidates varies across sentences. We study search utility through three quantities: total scaling gain, how much quality a sentence can gain from a much larger candidate pool; marginal scaling gain, the expected gain from generating one additional batch of candidates; and the sampling saturation point, the candidate budget required to realize most of the total scaling gain. We investigate two sources of information for predicting these quantities: signals available before candidate-set expansion, and statistics computed from the candidate pool accumulated during search. We find that sentence-level signals correlate with total scaling gain but are less informative about the sampling saturation point. In contrast, properties of the current candidate pool provide useful signals of marginal scaling gain. Finally, we show that these signals can identify sentences that obtain larger gains when additional search is selectively applied.

==> algorithms/marginal_gain_corrs.tex <==
\begin{algorithm}[h]
\small
\caption{Estimation of marginal gain correlations at budget $n$.}
\label{alg:marginal-corr}
\begin{algorithmic}[1]
\Require Candidate pools $\{C_i^{N_{\max}}\}_i$, decoder $d$,
evaluation metric $M$, predictor $f$, budget $n$,
number of resampling trials $R$
\For{each sentence $i$}
    \For{$r=1,\ldots,R$}
        \State Sample a random permutation of $C_i^{N_{\max}}$
        \State Construct nested pools:
        $C_i^{r,n/2} \subset C_i^{r,n} \subset C_i^{r,2n}$
        \State Decode and evaluate the pools at $n$ and $2n$
        to obtain $q_i^{d,r}(n)$ and $q_i^{d,r}(2n)$
        \State $\delta_i^r \gets
        q_i^{d,r}(2n) - q_i^{d,r}(n)$
        \If{$f = \mathrm{ObjStab}$}
            \State Get objectives
            $u_i^{d,r}(n/2)$ and $u_i^{d,r}(n)$
            \State $s_i^r \gets
            |u_i^{d,r}(n)-u_i^{d,r}(n/2)|$
        \Else
            \State $s_i^r \gets f(C_i^{r,n})$
        \EndIf
    \EndFor
    \State $\Delta_i^d(n,n)
        \gets \frac{1}{R}\sum_{r=1}^{R}\delta_i^r$
    \State $\bar{s}_i(n)
        \gets \frac{1}{R}\sum_{r=1}^{R}s_i^r$
\EndFor
\State $\rho \gets
\operatorname{Spearman}
\left(
\{\bar{s}_i(n)\}_i,
\{\Delta_i^d(n,n)\}_i
\right)$
\end{algorithmic}
\end{algorithm}

==> tables/qwen1b_lang_pairs.tex <==
\begin{table*}[!h]
\setlength{\fboxsep}{4.2pt}
\centering
\small
% Requires: \usepackage{booktabs,multirow,graphicx,colortbl,xcolor}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}

\begin{tabular}{llcccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{\textbf{en-es}} & \multicolumn{4}{c}{\textbf{en-de}} & \multicolumn{4}{c}{\textbf{en-ru}} \\
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
 &  & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
 &  & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ \\
\midrule


\multirow[c]{5}{*}{\rotatebox[origin=c]{90}{\textbf{Source-only}}} & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{diff.}}}} & \cellcolor{green!52} 0.33 & \cellcolor{green!44} 0.28 & \cellcolor{green!38} 0.24 & \cellcolor{green!27} 0.17 & \cellcolor{green!42} 0.27 & \cellcolor{green!49} 0.31 & \cellcolor{green!28} 0.18 & \cellcolor{green!24} 0.15 & \cellcolor{green!40} 0.25 & \cellcolor{green!49} 0.31 & \cellcolor{green!20} 0.13 & \cellcolor{green!30} 0.19 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{div.}}}} & \cellcolor{green!52} 0.33 & \cellcolor{green!37} 0.24 & \cellcolor{green!40} 0.25 & \cellcolor{green!27} 0.17 & \cellcolor{green!55} 0.35 & \cellcolor{green!47} 0.30 & \cellcolor{green!35} 0.22 & \cellcolor{green!23} 0.14 & \cellcolor{green!55} 0.35 & \cellcolor{green!51} 0.33 & \cellcolor{green!36} 0.23 & \cellcolor{green!37} 0.24 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{24}}}} & \cellcolor{green!41} 0.26 & \cellcolor{green!50} 0.32 & \cellcolor{green!28} 0.18 & \cellcolor{green!29} 0.18 & \cellcolor{green!34} 0.22 & \cellcolor{green!54} 0.34 & \cellcolor{green!22} 0.14 & \cellcolor{green!35} 0.22 & \cellcolor{green!33} 0.21 & \cellcolor{green!57} 0.36 & \cellcolor{green!11} 0.07 & \cellcolor{green!37} 0.23 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{25}}}} & \cellcolor{green!40} 0.25 & \cellcolor{green!48} 0.30 & \cellcolor{green!28} 0.18 & \cellcolor{green!24} 0.16 & \cellcolor{green!36} 0.23 & \cellcolor{green!51} 0.33 & \cellcolor{green!26} 0.16 & \cellcolor{green!33} 0.21 & \cellcolor{green!32} 0.20 & \cellcolor{green!50} 0.32 & \cellcolor{green!8} 0.05 & \cellcolor{green!28} 0.18 \\

 & {\colorbox{colorhex3_v2!80}{\makebox[1.3cm][l]{\tiny \srclen}}} & \cellcolor{green!19} 0.12 & \cellcolor{green!53} 0.34 & \cellcolor{green!9} 0.06 & \cellcolor{green!31} 0.20 & \cellcolor{green!21} 0.13 & \cellcolor{green!53} 0.34 & \cellcolor{green!15} 0.09 & \cellcolor{green!37} 0.24 & \cellcolor{green!19} 0.12 & \cellcolor{green!56} 0.36 & \cellcolor{green!5} 0.03 & \cellcolor{green!41} 0.26 \\

\cmidrule{1-14}

\multirow[c]{3}{*}{\rotatebox[origin=c]{90}{\;\;\;\; \textbf{Internal}}} & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \seqprob}}} & \cellcolor{green!92} 0.59 & \cellcolor{green!30} 0.19 & \cellcolor{green!63} 0.40 & \cellcolor{green!8} 0.05 & \cellcolor{green!76} 0.48 & \cellcolor{green!26} 0.17 & \cellcolor{green!55} 0.35 & \cellcolor{green!13} 0.08 & \cellcolor{green!76} 0.48 & \cellcolor{green!24} 0.16 & \cellcolor{green!46} 0.29 & \cellcolor{green!7} 0.04 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \surprisal}}} & \cellcolor{green!97} 0.62 & \cellcolor{green!32} 0.21 & \cellcolor{green!66} 0.42 & \cellcolor{green!8} 0.05 & \cellcolor{green!84} 0.53 & \cellcolor{green!31} 0.20 & \cellcolor{green!59} 0.38 & \cellcolor{green!14} 0.09 & \cellcolor{green!84} 0.53 & \cellcolor{green!28} 0.18 & \cellcolor{green!51} 0.33 & \cellcolor{green!10} 0.07 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \greedyent}}} & \cellcolor{green!100} \textbf{0.64} & \cellcolor{green!32} 0.20 & \cellcolor{green!71} 0.45 & \cellcolor{green!10} 0.06 & \cellcolor{green!91} 0.58 & \cellcolor{green!33} 0.21 & \cellcolor{green!65} 0.41 & \cellcolor{green!17} 0.11 & \cellcolor{green!88} 0.56 & \cellcolor{green!31} 0.20 & \cellcolor{green!54} 0.34 & \cellcolor{green!12} 0.08 \\

\bottomrule
\end{tabular}

\caption{
for \qwenthreeeone.
}
\label{tab:predictor-correlations}
\end{table*}

==> tables/qwen4b_lang_pairs.tex <==
\begin{table*}[!h]
\setlength{\fboxsep}{4.2pt}
\centering
\small
% Requires: \usepackage{booktabs,multirow,graphicx,colortbl,xcolor}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}

\begin{tabular}{llcccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{\textbf{en-es}} & \multicolumn{4}{c}{\textbf{en-de}} & \multicolumn{4}{c}{\textbf{en-ru}} \\
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
 &  & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
 &  & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ \\
\midrule


\multirow[c]{5}{*}{\rotatebox[origin=c]{90}{\textbf{Source-only}}} & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{diff.}}}} & \cellcolor{green!61} 0.40 & \cellcolor{green!37} 0.24 & \cellcolor{green!42} 0.28 & \cellcolor{green!11} 0.07 & \cellcolor{green!60} 0.40 & \cellcolor{green!52} 0.34 & \cellcolor{green!43} 0.29 & \cellcolor{green!21} 0.14 & \cellcolor{green!61} 0.40 & \cellcolor{green!40} 0.26 & \cellcolor{green!44} 0.29 & \cellcolor{green!29} 0.19 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{div.}}}} & \cellcolor{green!58} 0.38 & \cellcolor{green!40} 0.27 & \cellcolor{green!34} 0.22 & \cellcolor{green!12} 0.08 & \cellcolor{green!59} 0.39 & \cellcolor{green!53} 0.35 & \cellcolor{green!45} 0.30 & \cellcolor{green!21} 0.14 & \cellcolor{green!62} 0.41 & \cellcolor{green!41} 0.27 & \cellcolor{green!42} 0.28 & \cellcolor{green!26} 0.17 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{24}}}} & \cellcolor{green!58} 0.38 & \cellcolor{green!50} 0.33 & \cellcolor{green!40} 0.26 & \cellcolor{green!19} 0.12 & \cellcolor{green!53} 0.35 & \cellcolor{green!58} 0.38 & \cellcolor{green!38} 0.25 & \cellcolor{green!26} 0.17 & \cellcolor{green!54} 0.36 & \cellcolor{green!49} 0.32 & \cellcolor{green!34} 0.23 & \cellcolor{green!28} 0.19 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{25}}}} & \cellcolor{green!59} 0.39 & \cellcolor{green!45} 0.30 & \cellcolor{green!44} 0.29 & \cellcolor{green!20} 0.13 & \cellcolor{green!52} 0.34 & \cellcolor{green!55} 0.36 & \cellcolor{green!39} 0.26 & \cellcolor{green!27} 0.18 & \cellcolor{green!51} 0.34 & \cellcolor{green!41} 0.27 & \cellcolor{green!34} 0.22 & \cellcolor{green!23} 0.15 \\

 &  {\colorbox{colorhex3_v2!80}{\makebox[1.3cm][l]{\tiny \srclen}}}  & \cellcolor{green!35} 0.23 & \cellcolor{green!53} 0.35 & \cellcolor{green!11} 0.07 & \cellcolor{green!24} 0.16 & \cellcolor{green!34} 0.22 & \cellcolor{green!64} 0.42 & \cellcolor{green!21} 0.14 & \cellcolor{green!26} 0.17 & \cellcolor{green!33} 0.22 & \cellcolor{green!50} 0.33 & \cellcolor{green!18} 0.12 & \cellcolor{green!32} 0.21 \\

\cmidrule{1-14}

\multirow[c]{3}{*}{\rotatebox[origin=c]{90}{\;\;\;\; \textbf{Internal}}} & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \seqprob}}} & \cellcolor{green!84} 0.55 & \cellcolor{green!35} 0.23 & \cellcolor{green!47} 0.31 & \cellcolor{red!3} -0.02 & \cellcolor{green!89} 0.59 & \cellcolor{green!41} 0.27 & \cellcolor{green!53} 0.35 & \cellcolor{green!1} 0.01 & \cellcolor{green!80} 0.53 & \cellcolor{green!25} 0.17 & \cellcolor{green!53} 0.35 & \cellcolor{green!17} 0.11 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \surprisal}}} & \cellcolor{green!89} 0.58 & \cellcolor{green!38} 0.25 & \cellcolor{green!48} 0.32 & \cellcolor{red!2} -0.02 & \cellcolor{green!96} 0.63 & \cellcolor{green!44} 0.29 & \cellcolor{green!57} 0.38 & \cellcolor{green!3} 0.02 & \cellcolor{green!89} 0.59 & \cellcolor{green!30} 0.20 & \cellcolor{green!61} 0.40 & \cellcolor{green!19} 0.13 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \greedyent}}} & \cellcolor{green!93} 0.61 & \cellcolor{green!36} 0.23 & \cellcolor{green!51} 0.34 & \cellcolor{red!3} -0.02 & \cellcolor{green!100} \textbf{0.66} & \cellcolor{green!43} 0.28 & \cellcolor{green!62} 0.41 & \cellcolor{green!5} 0.03 & \cellcolor{green!93} 0.61 & \cellcolor{green!28} 0.18 & \cellcolor{green!64} 0.42 & \cellcolor{green!20} 0.13 \\


\bottomrule
\end{tabular}

\caption{
for \qwenthreeetwo.
}
\label{tab:predictor-correlations}
\end{table*}

==> tables/qwen8b_lang_pairs.tex <==
\begin{table*}[!h]
\setlength{\fboxsep}{4.2pt}
\centering
\small
% Requires: \usepackage{booktabs,multirow,graphicx,colortbl,xcolor}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}

\begin{tabular}{llcccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{\textbf{en-es}} & \multicolumn{4}{c}{\textbf{en-de}} & \multicolumn{4}{c}{\textbf{en-ru}} \\
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
 &  & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
 &  & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ \\
\midrule

\multirow[c]{5}{*}{\rotatebox[origin=c]{90}{\textbf{Source-only}}} & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{diff.}}}}  & \cellcolor{green!69} 0.43 & \cellcolor{green!41} 0.26 & \cellcolor{green!47} 0.29 & \cellcolor{green!21} 0.13 & \cellcolor{green!66} 0.41 & \cellcolor{green!38} 0.24 & \cellcolor{green!44} 0.27 & \cellcolor{green!15} 0.10 & \cellcolor{green!64} 0.40 & \cellcolor{green!44} 0.28 & \cellcolor{green!35} 0.22 & \cellcolor{green!11} 0.07 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{div.}}}} & \cellcolor{green!60} 0.37 & \cellcolor{green!49} 0.31 & \cellcolor{green!30} 0.19 & \cellcolor{green!14} 0.09 & \cellcolor{green!59} 0.37 & \cellcolor{green!44} 0.28 & \cellcolor{green!39} 0.25 & \cellcolor{green!11} 0.07 & \cellcolor{green!47} 0.30 & \cellcolor{green!39} 0.25 & \cellcolor{green!19} 0.12 & \cellcolor{green!18} 0.11 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{24}}}} & \cellcolor{green!68} 0.42 & \cellcolor{green!58} 0.36 & \cellcolor{green!42} 0.26 & \cellcolor{green!22} 0.14 & \cellcolor{green!54} 0.34 & \cellcolor{green!48} 0.30 & \cellcolor{green!34} 0.21 & \cellcolor{green!22} 0.14 & \cellcolor{green!54} 0.34 & \cellcolor{green!48} 0.30 & \cellcolor{green!24} 0.15 & \cellcolor{green!12} 0.08 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{25}}}} & \cellcolor{green!67} 0.42 & \cellcolor{green!59} 0.37 & \cellcolor{green!42} 0.26 & \cellcolor{green!18} 0.11 & \cellcolor{green!54} 0.34 & \cellcolor{green!42} 0.26 & \cellcolor{green!36} 0.22 & \cellcolor{green!21} 0.13 & \cellcolor{green!53} 0.33 & \cellcolor{green!44} 0.28 & \cellcolor{green!25} 0.16 & \cellcolor{green!10} 0.06 \\

 & {\colorbox{colorhex3_v2!80}{\makebox[1.3cm][l]{\tiny \srclen}}} & \cellcolor{green!43} 0.27 & \cellcolor{green!70} 0.43 & \cellcolor{green!12} 0.08 & \cellcolor{green!21} 0.13 & \cellcolor{green!26} 0.16 & \cellcolor{green!56} 0.35 & \cellcolor{green!16} 0.10 & \cellcolor{green!27} 0.17 & \cellcolor{green!12} 0.08 & \cellcolor{green!52} 0.32 & \cellcolor{red!9} -0.05 & \cellcolor{green!17} 0.11 \\

\cmidrule{1-14}

\multirow[c]{3}{*}{\rotatebox[origin=c]{90}{\;\;\;\; \textbf{Internal}}} & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \seqprob}}} & \cellcolor{green!75} 0.47 & \cellcolor{green!33} 0.21 & \cellcolor{green!44} 0.27 & \cellcolor{green!14} 0.09 & \cellcolor{green!91} 0.57 & \cellcolor{green!31} 0.19 & \cellcolor{green!59} 0.37 & \cellcolor{green!20} 0.13 & \cellcolor{green!85} 0.53 & \cellcolor{green!29} 0.18 & \cellcolor{green!48} 0.30 & \cellcolor{green!1} 0.01 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \surprisal}}} & \cellcolor{green!79} 0.49 & \cellcolor{green!34} 0.21 & \cellcolor{green!44} 0.28 & \cellcolor{green!13} 0.08 & \cellcolor{green!96} 0.60 & \cellcolor{green!36} 0.22 & \cellcolor{green!63} 0.39 & \cellcolor{green!21} 0.13 & \cellcolor{green!91} 0.57 & \cellcolor{green!30} 0.19 & \cellcolor{green!50} 0.31 & \cellcolor{green!1} 0.01 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \greedyent}}} & \cellcolor{green!80} 0.50 & \cellcolor{green!28} 0.18 & \cellcolor{green!48} 0.30 & \cellcolor{green!14} 0.09 & \cellcolor{green!100} \textbf{0.62} & \cellcolor{green!32} 0.20 & \cellcolor{green!66} 0.41 & \cellcolor{green!20} 0.12 & \cellcolor{green!93} 0.58 & \cellcolor{green!29} 0.18 & \cellcolor{green!54} 0.34 & \cellcolor{green!2} 0.01 \\



\bottomrule
\end{tabular}

\caption{
for \qwenthreeethree.
}
\label{tab:predictor-correlations}
\end{table*}

==> tables/tower2b_lang_pairs.tex <==
\begin{table*}[!h]
\setlength{\fboxsep}{4.2pt}
\centering
\small
% Requires: \usepackage{booktabs,multirow,graphicx,colortbl,xcolor}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}

\begin{tabular}{llcccccccccccc}
\toprule
 &  & \multicolumn{4}{c}{\textbf{en-es}} & \multicolumn{4}{c}{\textbf{en-de}} & \multicolumn{4}{c}{\textbf{en-ru}} \\
\cmidrule(lr){3-6}
\cmidrule(lr){7-10}
\cmidrule(lr){11-14}
 &  & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} & \multicolumn{2}{c}{\textbf{MBR}} & \multicolumn{2}{c}{\textbf{Reranking}} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
\cmidrule(lr){13-14}
 &  & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ & \shortstack{$\rho_G$} & $\rho_{N^{\text{.95}}}$ \\
\midrule

\multirow[c]{5}{*}{\rotatebox[origin=c]{90}{\textbf{Source-only}}} & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{diff.}}}} & \cellcolor{green!47} 0.33 & \cellcolor{green!37} 0.26 & \cellcolor{green!40} 0.28 & \cellcolor{green!11} 0.08 & \cellcolor{green!52} 0.37 & \cellcolor{green!43} 0.30 & \cellcolor{green!38} 0.27 & \cellcolor{green!20} 0.14 & \cellcolor{green!47} 0.33 & \cellcolor{green!38} 0.27 & \cellcolor{green!33} 0.23 & \cellcolor{green!17} 0.12 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \precomet\textsubscript{div.}}}} & \cellcolor{green!26} 0.18 & \cellcolor{green!35} 0.25 & \cellcolor{green!27} 0.19 & \cellcolor{green!9} 0.06 & \cellcolor{green!36} 0.25 & \cellcolor{green!43} 0.30 & \cellcolor{green!31} 0.22 & \cellcolor{green!20} 0.14 & \cellcolor{green!23} 0.16 & \cellcolor{green!30} 0.21 & \cellcolor{green!21} 0.15 & \cellcolor{green!13} 0.09 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{24}}}} & \cellcolor{green!35} 0.24 & \cellcolor{green!46} 0.33 & \cellcolor{green!35} 0.25 & \cellcolor{green!17} 0.12 & \cellcolor{green!37} 0.26 & \cellcolor{green!43} 0.30 & \cellcolor{green!30} 0.21 & \cellcolor{green!22} 0.15 & \cellcolor{green!35} 0.25 & \cellcolor{green!40} 0.28 & \cellcolor{green!23} 0.16 & \cellcolor{green!17} 0.12 \\

 & {\colorbox{colorhex2_v2}{\makebox[1.3cm][l]{\tiny \sentinel\textsubscript{25}}}} & \cellcolor{green!40} 0.28 & \cellcolor{green!44} 0.31 & \cellcolor{green!33} 0.23 & \cellcolor{green!14} 0.10 & \cellcolor{green!39} 0.27 & \cellcolor{green!47} 0.33 & \cellcolor{green!27} 0.19 & \cellcolor{green!19} 0.13 & \cellcolor{green!39} 0.27 & \cellcolor{green!37} 0.26 & \cellcolor{green!22} 0.15 & \cellcolor{green!13} 0.09 \\

 & {\colorbox{colorhex3_v2!80}{\makebox[1.3cm][l]{\tiny \srclen}}} & \cellcolor{red!23} -0.16 & \cellcolor{green!37} 0.26 & \cellcolor{green!3} 0.02 & \cellcolor{green!24} 0.16 & \cellcolor{red!15} -0.11 & \cellcolor{green!41} 0.29 & \cellcolor{red!3} -0.02 & \cellcolor{green!19} 0.14 & \cellcolor{red!23} -0.16 & \cellcolor{green!35} 0.25 & \cellcolor{red!17} -0.12 & \cellcolor{green!15} 0.10 \\

\cmidrule{1-14}

\multirow[c]{4}{*}{\rotatebox[origin=c]{90}{\;\;\;\; \textbf{Internal}}} & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \seqprob}}} & \cellcolor{green!92} 0.64 & \cellcolor{green!27} 0.19 & \cellcolor{green!47} 0.33 & \cellcolor{red!3} -0.02 & \cellcolor{green!88} 0.62 & \cellcolor{green!26} 0.18 & \cellcolor{green!57} 0.40 & \cellcolor{green!4} 0.03 & \cellcolor{green!87} 0.61 & \cellcolor{green!10} 0.07 & \cellcolor{green!63} 0.44 & \cellcolor{green!2} 0.02 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \surprisal}}} & \cellcolor{green!96} 0.68 & \cellcolor{green!29} 0.21 & \cellcolor{green!50} 0.35 & \cellcolor{red!4} -0.03 & \cellcolor{green!95} 0.67 & \cellcolor{green!27} 0.19 & \cellcolor{green!63} 0.44 & \cellcolor{green!3} 0.02 & \cellcolor{green!93} 0.65 & \cellcolor{green!11} 0.08 & \cellcolor{green!65} 0.46 & \cellcolor{green!3} 0.02 \\

 & {\colorbox{colorhex1_v2}{\makebox[1.3cm][l]{\tiny \greedyent}}} & \cellcolor{green!100} 0.70 & \cellcolor{green!23} 0.16 & \cellcolor{green!51} 0.36 & \cellcolor{red!4} -0.03 & \cellcolor{green!100} \textbf{0.70} & \cellcolor{green!24} 0.17 & \cellcolor{green!65} 0.46 & \cellcolor{green!1} 0.00 & \cellcolor{green!96} 0.67 & \cellcolor{green!9} 0.07 & \cellcolor{green!68} 0.48 & \cellcolor{green!2} 0.02 \\

\bottomrule
\end{tabular}

\caption{
for \towertwob.
}
\label{tab:predictor-correlations}
\end{table*}
